Discovering the Skyline of Web Databases

Many web databases are "hidden" behind proprietary search interfaces that enforce the top-$k$ output constraint, i.e., each query returns at most $k$ of all matching tuples, preferentially selected and returned according to a proprietary ranking function. In this paper, we initiate research into the novel problem of skyline discovery over top-$k$ hidden web databases. Since skyline tuples provide critical insights into the database and include the top-ranked tuple for every possible ranking function following the monotonic order of attribute values, skyline discovery from a hidden web database can enable a wide variety of innovative third-party applications over one or multiple web databases. Our research in the paper shows that the critical factor affecting the cost of skyline discovery is the type of search interface controls provided by the website. As such, we develop efficient algorithms for three most popular types, i.e., one-ended range, free range and point predicates, and then combine them to support web databases that feature a mixture of these types. Rigorous theoretical analysis and extensive real-world online and offline experiments demonstrate the effectiveness of our proposed techniques and their superiority over baseline solutions.

==> lowerboundproof.tex <==
\newtheorem{theorem}{Theorem}
\begin{theorem} \label{thm:ner}
Considering the SQ interface, there exists a database such that discovering its skyline requires more than $(m-1)(|S|-1)^{m-1}$ queries.
\end{theorem}
\begin{proof}
Without loss of generality, consider a database with $m$ attribute $A_1$ to $A_m$ with a Top-$1$ query interface. Suppose the database has only two skyline tuples: $t_1=\langle 0.1,1,1,\dots , 1\rangle$ and $t_2=\langle 1,0.1,0.1,\dots , 0.1\rangle$.
At least one query is required to discover the first skyline tuple, let us say $t_1$ (the proof is similar for the case where the first discovered tuple is $t_2$). In order to make sure all the skylines are discovered, one needs to check the following $m$ areas:
\begin{itemize}
\item $q_1: A_1<0.1$
\item $q_2: A_1\geq 0.1$ AND $A_2<1$ 
\item $q_3: A_1\geq 0.1$ AND $A_2\geq 1$ AND $A_3<1$ 
\item $\dots$
\item $q_m: A_1\geq 0.1$ AND $A_2\geq 1$ AND $\dots$ AND $A_m<1$ 
\end{itemize}
$q_1$ returns empty. The optimal algorithm should select one of the remaining queries (or a subset of them) and issue it (We note that different ordering of the attributes partitions the area in different queries, but still the number of queries and the rest of proof will not change).
Suppose the optimal algorithm issues the query $q_i: A_1\geq 0.1$ AND $\dots$ AND $A_i<1$. $\forall j>1,$ $j\neq i$, the algorithm needs to check the regions fall into $q_j$ and are not dominated by $t_2$. We note that if it simply issues $q_j$, it returns $t_2$ that will not help. Therefore, for each such $j$, similar to $q_1$ to $q_m$, the algorithm needs to issue $m$ queries (no matter in which order) to confirm the emptiness of those regions. Consequently, for this database, any algorithm needs more than $(m-1)(|S|-1)^{m-1}$ queries.
\end{proof}

==> oldexp.tex <==
\section{Experimental Evaluation}
\label{sec:experiments}

%%%%%%%%%%%%%Note: no skyband experiments. we will remove the mention from sec 7


\subsection{Experimental Setup}

\noindent {\bf Datasets:} We tested two real-world databases in our experiments:  One is an offline experiment on the flight on-time statistics database published by the US Department of Transportation (DOT).  It contains the delay and other scheduling information, such as scheduled and actual departure time, taxing time and other detailed delay metrics, for all flights conducted by the 14 US carriers. The dataset has been widely used by third party websites to identify the on-time performance of flights, routes, airports, airlines, etc.

We used the complete dataset for the month of May, 2015\footnote{downloaded from \url{http://www.transtats.bts.gov/DL_SelectFields.asp?Table_ID=236&DB_Short_Name=On-Time}}.  It consisted of 457,013 tuples and 28 attributes, from which we chose a subset of 9 ordinal attributes as {\em ranking attributes} (the other attributes, such as Flight Number, are considered filtering attributes).  These 9 attributes chosen are \textit{Dep-Delay, Taxi-out, Taxi-in, Actual-elapsed-time, Air-time, Distance, Delay-group-normal, Distance-group, ArrivalDelay}.  To test databases with varying sizes, we drew uniform random samples from the dataset to form database with a given size.

The domain of the 9 ranking attributes range from 11 to 4,983.  Since only two of the 9 attributes, \textit{Delay-group-normal} and \textit{Distance-group}, are properly discretized (i.e., ``grouped'', according to the dataset description) for use as a PQ (point-query-predicate) attribute, when our experiments call for more PQ attributes, we consider four other derived attributes, \textit{Taxi-out group, Taxi-in group, ArrivalDelay group, Air-Time group} as potential PQ attributes. The other attributes are treated as range-predicate attributes - whether it is SQ or RQ depends on the specific experimental setup.

For all attributes, the preferential order is defined so that shorter delay/duration is ranked higher than longer values. For non-time attributes, i.e., \textit{Distance} and \textit{Distance-group}, we assign a higher rank to longer distances than shorter ones - e.g., a motivation here is in the interest of travelers who want to accumulate more miles while spending as little time/delay as possible.

To properly run the dataset as a web database, we also need to define a ranking function used by the database. To this end, we used the SUM of all attributes minus the \textit{distance} (or distance-group) as the ranking function (preferring tuples with a small output). While the value of $k$ (as in top-$k$ interface) used by the hidden database does not affect the performance of our algorithm at all, we nevertheless make the most conservative setting of $k = 1$ in all tests.

Another real-world hidden database we tested is through a {\bf live online experiment} on Google Flights (GF), which is an online booking service that offers a limited API search interface called QPX API\footnote{\url{https://developers.google.com/qpx-express/}}.  We considered one filtering attribute, the departure city, and four ranking attributes supported by the API: {\em Stops}, {\em Price}, {\em ConnectionDuration}, and {\em DepartureTime}. Specifically, QPX API supports SQ (i.e., single-ended ranges) on the first three attributes - specifically, through API parameters maxStops, maxPrice and maxConnectionDuration - and RQ (i.e., two-ended) on DepartureTime through a (range) parameter PermittedDepartureTime. QPX API defaults to rank by price (low to high).

On these four attributes, we consider a ranking order that prefers fewer {\em Stops}, lower {\em Price}, shorter {\em ConnectionDuration}, and earlier {\em DepartureTime}, conditioning upon the filtering attributes of departure city and arrival city.  Imagine a leisure traveler who wants to get away by flying from one city to another.  The traveler generally prefers a shorter non-stop flight, a lower price, and to get away as early as possible so as to take full advantage of the vacation day.  The skyline tuples (i.e., flights) discovered through our live experiment exactly serves the need of such a traveler.

\vspace{1mm}
\noindent {\bf Algorithms Evaluated:}
We tested $4$ algorithms described in the paper:
SQ-DB-CRAWL,  RQ-DB-CRAWL and PQ-DB-CRAWL corresponding to the homogeneous search interfaces
with SQ, RQ and PQ predicates, respectively; and MQ-DB-CRAWL which supports a mixture of all predicates.

\vspace{1mm}
\noindent {\bf Performance Measures:}
Since all our algorithms are guaranteed to discover all skyline tuples,
we focused on the measuring the query cost - i.e., the number of queries issued to the database.

\begin{figure*}[ht]
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        %\includegraphics[width = 40mm]{plots/RQ-N.pdf}
        \includegraphics[scale=0.26]{plots/RQ-N.pdf}
        \vspace{-2mm}\caption{Range Predicates: Impact of $n$}
        \label{fig:rq-n}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/RQ-D.pdf}
        \vspace{-2mm}\caption{Range Predicates: Impact of $m$}
        \label{fig:rq-m}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/PQ-N.pdf}
        \vspace{-2mm}\caption{Point Predicates: Impact of $n$}
        \label{fig:pq-n}
    \end{minipage}
    \hspace{3mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/PQ-D.pdf}
        \vspace{-2mm}\caption{Point Predicates: Impact of $m$}
        \label{fig:pq-m}
    \end{minipage}
    \hspace{-2mm}
\end{figure*}
\begin{figure*}[ht]
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        %\includegraphics[width = 40mm]{plots/RQ-N.pdf}
        \includegraphics[scale=0.26]{plots/PQ-SD.pdf}
        \vspace{-2mm}\caption{Point Predicates: Impact of Domain Size}
        \label{fig:pq-sd}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/MQ-N.pdf}
        \vspace{-2mm}\caption{Mixed Predicates: Impact of $n$}
        \label{fig:mq-n}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/MQ-DR.pdf}
        \vspace{-2mm}\caption{Mixed Predicates: Varying Range Predicates}
        \label{fig:mq-dr}
    \end{minipage}
    \hspace{3mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/MQ-DP.pdf}
        \vspace{-2mm}\caption{Mixed Predicates: Varying Point Predicates}
        \label{fig:mq-dp}
    \end{minipage}
    \hspace{-2mm}
\end{figure*}
\begin{figure*}[ht]
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/template.pdf}
        \vspace{-2mm}\caption{Tradeoff for MIXED-DB-CRAWL}
        \label{fig:mq-tradeoff}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/RQ-Progress.pdf}
        \vspace{-2mm}\caption{Anytime Property of SQ and RQ-DB-CRAWL}
        \label{fig:rq-anytime}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/PQ-Progress.pdf}
        \vspace{-2mm}\caption{Anytime Property of PQ-DB-CRAWL}
        \label{fig:pq-anytime}
    \end{minipage}
    \hspace{1mm}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[scale=0.26]{plots/onlineExp1.pdf}
        \vspace{-2mm}\caption{Online Experiment}
        \label{fig:onlineExp1}
    \end{minipage}
    \hspace{-2mm}
\end{figure*}

\subsection{Experimental Results}

\textcolor{red}{1. Please remove RQ-DB-Mixed lines from the figures\\}
\textcolor{red}{2. Please make sure no legend covers lines in the figures}

\noindent {\bf Interfaces with Range Predicates:}
We started with testing skyline discovery through range-query interfaces, i.e., SQ and RQ, over the DOT dataset. Figure~\ref{fig:rq-n} shows the query cost of SQ- and RQ-DB-CRAWL when the database size ranges from 20K to 100K.  The figure also depicts how the number of skyline tuples $|S|$ varies in these databases. One can observe from the figure that RQ-DB-CRAWL is more efficient than its SQ- counterpart as it leverages the more powerful, two-ended, search interface. In addition, there is also an interesting observation on how the query cost changes with the database size $n$: With SQ-DB-CRAWL, the query cost does {\em not} increase with $n$, but rather depends heavily on the number of skyline tuples $|S|$. On the other hand, RQ-DB-CRAWL does incur a generally higher query cost when $n$ increases. Both are consistent with our theoretical analysis in \textcolor{red}{Section~\ref{}}.

Figure~\ref{fig:rq-m} shows the result of varying the number of attributes. Once again, RQ- outperforms SQ-DB-CRAWL. While the query costs for both do increase with a higher dimensionality, (at least) partially because the number of skyline tuples also increases rapidly with dimensionality \cite{buchta1989average}, the query cost for skyline crawling remains small even when the number of range attributes reaches 6.

Another important observation from both figures is that our techniques outperform the baseline method discussed in the introduction - i.e., crawling all tuples first before computing the skyline offline - by orders of magnitude. Specifically, note that any database-crawling based method requires at the very least $n/k$ tuples, because each query returns at most $k$ tuples. The query costs reported in both figures, and indeed in all remaining figures in this section, are orders of magnitude smaller than $n/k$, which in this case is at least in the order of $10^4$ in all experiments.

\vspace{1mm}
\noindent {\bf Interfaces with Point Predicates:}
In the next set of experiments, we tested PQ-DB-CRAWL. Figure~\ref{fig:pq-n} shows how the query cost varies with $n$ and $m$.  One can see that, while the query cost is barely affected by $n$, it does increase significantly with a larger $m$ - as predicted by our theoretical analysis in \textcolor{red}{Section~\ref{}}. In Figure~\ref{fig:pq-sd}, we further tested how the query cost changes with varying domain sizes. In this experiment, for a fixed domain size (from $v = $ 5 to 15), we first select all PQ attributes with domain larger than $v$, and then remove from the domain all but $v$ values (all tuples associated with these values are also removed). Then, we select 100,000 tuples from the remaining tuples as our testing database. One can see from the result that, while larger attribute domains do lead to a higher query cost, the increase on query cost is not nearly as fast as the data space (which grows with $v^m$) - indicating the scalability of our algorithm to larger attribute domains.

\vspace{1mm}
\noindent {\bf Interfaces with Mixed Predicates:}
We next evaluated the more realistic search interfaces that contain a mixture of range and point predicates. In the first experiment, we considered 3 RQ and 2 PQ predicates and evaluated how the query cost varies with database size. Figure~\ref{fig:mq-n} shows that, as expected, the number of tuples only have minimal impact on query cost. In the next test, we considered how varying number of RQ and PQ attributes affect the performance of MQ-DB-CRAWL. Specifically, the two lines in Figure~\ref{fig:mq-dr} represent the following two cases: (1) 1 PQ attribute with the number of RQ attributes varying from 2 to 5, and (2) 1 RQ attribute with the number of PQ ones from 2 to 5.  We can observe from the figure that the impact on query cost is much more pronounced on an increase of the number of PQ attributes - consistent with our discussions earlier in the paper.

\vspace{1mm}
\noindent {\bf Anytime Property of Skyline Discovery:}
Recall from \textcolor{red}{Appendix~\ref{sec:extensions}} that all the algorithms in our paper share the anytime property 
- i.e., one can stop the algorithm execution at any time to return a  subset of all skyline tuples.
Figures~\ref{fig:rq-anytime} and \ref{fig:pq-anytime} trace the progress of our algorithms in a crawling case of $100 k$ tuples (there are $5$ predicates in RQ-DB, and $4$ in PQ-DB case)
and measure the cumulative query cost as they systematically discover new skylines.
In Figures~\ref{fig:rq-anytime}, in addition to SQ-DB-Crawl and RQ-DB-Crawl, we added a trend for the intermediate RQ-DB skyline crawling method. SQ-DB-Crawl could find the first 16 skylines without facing a skyline twice, which ended in having the maximum performance up to that point (performing better than the intermediate method); however, discovering the same skyline point multiple times, it lost its cost minimality, and at point 24, the intermediate method outperformed it. On the other hand, changing the crawling strategy after facing a discovered skyline helped RQ-DB-Crwal to maintain its query cost low.
Figure~\ref{fig:pq-anytime} shows that despite the limitations of point query interface the algorithm could discover all the skyline points with less than 600 queries. The peak between the $8^{th}$ and $9^{th}$ skylines, in this case, is because of the queries spent for crawling the areas that did not contain any skyline tuple.

\vspace{1mm}
\noindent {\bf Skyline Discovery over Google Flights:}
Our experiment setup is as follows. We randomly chose a pair of airports from top-25 busiest airports in USA and a date between August 1 and 31, 2015, and sought to find all the skyline flights on that day. We repeated this process for 50 different pairs and reported the average query cost. The number of skyline flights varied between 4 to 11.  We invoke the MQ-DB-CRAWL algorithm for this purpose and Figure~\ref{fig:onlineExp1} shows the results. We verified the correctness of the results by crawling all the flights for the same date and comparing the results. One can observe that our algorithm is highly efficient - being able to discover all skyline tuples within a query cost lower than 50, which is the (free) rate limit imposed per user account per day by Google QPX API.

